Dynamically Tagged Groups of Metal-Poor Stars from the Best \& Brightest Survey

Orbital characteristics based on Gaia Early Data Release 3 astrometric parameters are analyzed for ${\sim} 4000$ metal-poor stars ([Fe/H] $\leq -0.8$) compiled from the Best $\&$ Brightest survey. Selected as metal-poor candidates based on broadband near- and far-IR photometry, $43\%$ of these stars had medium-resolution ($1200 \lesssim R \lesssim 2000$) validation spectra obtained over a seven-year campaign from $2014$ to $2020$ with a variety of telescopes. The remaining stars were chosen based on photometric metallicity determinations from the Huang et al. recalibration of the Sky Mapper Southern Survey. Dynamical clusters of these stars are obtained from the orbital energy and cylindrical actions using the \HDBSCAN ~unsupervised learning algorithm. We identify $52$ Dynamically Tagged Groups (DTGs) with between $5$ and $21$ members; $18$ DTGs have at least $10$ member stars. Milky Way (MW) substructures such as Gaia-Sausage-Enceladus, the Metal-Weak Thick-Disk, Thamnos, the Splashed Disk, and the Helmi Stream are identified. Associations with MW globular clusters are determined for $8$ DTGs; no recognized MW dwarf galaxies were associated with any of our DTGs. Previously identified dynamical groups are also associated with our DTGs, with emphasis placed on their structural determination and possible new identifications. Chemically peculiar stars are identified as members of several DTGs, with $6$ DTGs that are associated with \textit{r}-process-enhanced stars. We demonstrate that the mean carbon and $\alpha$-element abundances of our DTGs are correlated with their mean metallicity in an understandable manner. Similarly, we find that the mean metallicity, carbon, and $\alpha$-element abundances are separable into different regions of the mean rotational-velocity space.

==> Tables/cluster_orbital_table.tex <==
\startlongtable
\begin{deluxetable*}{l  r  c  c  r  r}
\tablecaption{Cluster Dynamical Parameters Determined by \AGAMA \label{tab:cluster_orbit}}
\tablehead{\colhead{Cluster} & \colhead{$N$ Stars} & \colhead{($\langle$v$_{\text{r}}\rangle$,$\langle$v$_{\phi}\rangle$,$\langle$v$_{\text{z}}\rangle$)} & \colhead{($\langle$J$_{\text{r}}\rangle$,$\langle$J$_{\phi}\rangle$,$\langle$J$_{\text{z}}\rangle$)} & \colhead{$\langle$E$\rangle$} & \colhead{$\langle$ecc$\rangle$}\\
\colhead{} & \colhead{} & \colhead{($\sigma_{\langle\text{v}_{\text{r}}\rangle}$,$\sigma_{\langle\text{v}_{\phi}\rangle}$,$\sigma_{\langle\text{v}_{\text{z}}\rangle}$)} & \colhead{($\sigma_{\langle\text{J}_{\text{r}}\rangle}$,$\sigma_{\langle\text{J}_{\phi}\rangle}$,$\sigma_{\langle\text{J}_{\text{z}}\rangle}$)} & \colhead{$\sigma_{\langle\text{E}\rangle}$} & \colhead{$\sigma_{\langle\text{ecc}\rangle}$}\\
\colhead{} & \colhead{} & \colhead{(km s$^{-1}$)} & \colhead{(kpc km s$^{-1}$)} & \colhead{(10$^{5}$ km$^{2}$ s$^{-2}$)} & \colhead{}}
\startdata
$DTG-1$ & $21$ & ($0.8$,$216.2$,$-1.0$) & ($10.3$,$1749.2$,$2.3$) & $-1.603$ & $0.090$ \\
 & & ($21.3$,$7.4$,$15.0$) & ($5.9$,$29.8$,$2.4$) & $0.007$ & $0.026$ \\
$DTG-2$ & $20$ & ($12.7$,$124.0$,$-21.8$) & ($163.5$,$936.0$,$273.8$) & $-1.664$ & $0.421$ \\
 & & ($90.4$,$37.1$,$106.0$) & ($75.7$,$219.9$,$26.7$) & $0.036$ & $0.113$ \\
$DTG-3$ & $18$ & ($23.7$,$4.8$,$0.5$) & ($894.7$,$45.8$,$58.5$) & $-1.644$ & $0.932$ \\
 & & ($153.2$,$13.0$,$38.5$) & ($48.5$,$120.4$,$17.9$) & $0.028$ & $0.040$ \\
$DTG-4$ & $18$ & ($-22.4$,$-14.0$,$-81.0$) & ($159.5$,$-80.7$,$1032.0$) & $-1.661$ & $0.443$ \\
 & & ($133.1$,$39.9$,$143.3$) & ($69.7$,$182.7$,$96.0$) & $0.052$ & $0.104$ \\
$DTG-5$ & $17$ & ($-40.7$,$67.4$,$-4.6$) & ($447.1$,$492.3$,$69.5$) & $-1.765$ & $0.733$ \\
 & & ($103.8$,$21.2$,$58.2$) & ($59.9$,$118.8$,$17.6$) & $0.022$ & $0.062$ \\
$DTG-6$ & $15$ & ($-23.8$,$10.3$,$-10.1$) & ($267.2$,$71.7$,$1802.0$) & $-1.392$ & $0.398$ \\
 & & ($110.3$,$40.5$,$256.0$) & ($195.0$,$352.5$,$151.0$) & $0.052$ & $0.164$ \\
$DTG-7$ & $13$ & ($-79.9$,$13.6$,$33.4$) & ($1259.4$,$97.7$,$174.9$) & $-1.452$ & $0.945$ \\
 & & ($289.7$,$20.2$,$115.0$) & ($69.2$,$160.4$,$21.5$) & $0.030$ & $0.022$ \\
$DTG-8$ & $12$ & ($-100.7$,$11.2$,$34.2$) & ($1167.6$,$92.3$,$293.3$) & $-1.454$ & $0.956$ \\
 & & ($269.4$,$13.2$,$129.4$) & ($135.8$,$105.9$,$26.5$) & $0.044$ & $0.035$ \\
$DTG-9$ & $12$ & ($42.0$,$109.8$,$-131.9$) & ($121.5$,$655.2$,$196.1$) & $-1.831$ & $0.437$ \\
 & & ($9.7$,$12.6$,$9.3$) & ($14.3$,$48.1$,$19.7$) & $0.009$ & $0.027$ \\
$DTG-10$ & $12$ & ($-96.5$,$8.5$,$5.7$) & ($976.8$,$82.9$,$135.9$) & $-1.563$ & $0.962$ \\
 & & ($170.9$,$14.9$,$76.1$) & ($67.6$,$126.7$,$17.7$) & $0.018$ & $0.019$ \\
$DTG-11$ & $12$ & ($-6.6$,$11.7$,$11.9$) & ($550.2$,$52.9$,$298.4$) & $-1.721$ & $0.925$ \\
 & & ($179.4$,$23.3$,$105.1$) & ($38.4$,$111.4$,$41.8$) & $0.019$ & $0.049$ \\
$DTG-12$ & $11$ & ($-4.1$,$186.1$,$1.1$) & ($64.3$,$1506.9$,$3.8$) & $-1.657$ & $0.236$ \\
 & & ($45.2$,$6.2$,$18.9$) & ($10.2$,$29.6$,$2.6$) & $0.006$ & $0.019$ \\
$DTG-13$ & $11$ & ($-20.3$,$255.1$,$2.4$) & ($24.2$,$2136.1$,$1.0$) & $-1.491$ & $0.126$ \\
 & & ($17.8$,$4.2$,$11.6$) & ($6.7$,$14.0$,$1.1$) & $0.004$ & $0.018$ \\
$DTG-14$ & $11$ & ($-25.9$,$168.7$,$25.8$) & ($58.7$,$953.9$,$74.8$) & $-1.825$ & $0.277$ \\
 & & ($48.0$,$25.4$,$37.1$) & ($26.6$,$67.5$,$15.6$) & $0.028$ & $0.066$ \\
$DTG-15$ & $10$ & ($-19.0$,$75.1$,$-44.0$) & ($265.0$,$397.7$,$102.2$) & $-1.904$ & $0.687$ \\
 & & ($109.0$,$23.2$,$64.9$) & ($40.0$,$104.5$,$13.5$) & $0.027$ & $0.075$ \\
$DTG-16$ & $10$ & ($-22.1$,$62.5$,$37.2$) & ($357.0$,$408.0$,$34.6$) & $-1.886$ & $0.732$ \\
 & & ($61.9$,$15.4$,$7.1$) & ($47.8$,$101.8$,$12.8$) & $0.022$ & $0.067$ \\
$DTG-17$ & $9$ & ($19.3$,$9.9$,$13.4$) & ($538.5$,$68.0$,$91.6$) & $-1.863$ & $0.911$ \\
 & & ($68.1$,$8.7$,$63.1$) & ($43.7$,$56.5$,$4.9$) & $0.028$ & $0.088$ \\
$DTG-18$ & $9$ & ($29.8$,$21.1$,$17.4$) & ($762.1$,$164.5$,$102.1$) & $-1.677$ & $0.902$ \\
 & & ($150.0$,$14.7$,$52.3$) & ($28.2$,$131.3$,$11.4$) & $0.005$ & $0.038$ \\
$DTG-19$ & $9$ & ($-19.5$,$171.6$,$-1.8$) & ($96.3$,$1398.5$,$4.2$) & $-1.675$ & $0.294$ \\
 & & ($59.4$,$4.5$,$19.5$) & ($11.2$,$20.7$,$2.1$) & $0.004$ & $0.018$ \\
\pagebreak
$DTG-20$ & $8$ & ($-12.6$,$87.7$,$-4.8$) & ($457.2$,$737.2$,$20.5$) & $-1.714$ & $0.673$ \\
 & & ($126.6$,$12.7$,$34.8$) & ($26.1$,$43.3$,$10.9$) & $0.011$ & $0.018$ \\
$DTG-21$ & $8$ & ($52.2$,$32.1$,$-28.5$) & ($392.5$,$184.7$,$67.1$) & $-1.935$ & $0.789$ \\
 & & ($70.6$,$8.8$,$36.8$) & ($32.8$,$49.6$,$12.8$) & $0.012$ & $0.042$ \\
$DTG-22$ & $8$ & ($-66.2$,$36.2$,$19.9$) & ($658.5$,$264.8$,$47.9$) & $-1.729$ & $0.866$ \\
 & & ($157.2$,$8.7$,$32.7$) & ($25.2$,$60.9$,$17.8$) & $0.039$ & $0.038$ \\
$DTG-23$ & $8$ & ($-1.2$,$223.9$,$-4.6$) & ($2.4$,$1855.9$,$0.7$) & $-1.576$ & $0.042$ \\
 & & ($6.8$,$2.6$,$5.1$) & ($1.2$,$8.1$,$0.4$) & $0.002$ & $0.012$ \\
$DTG-24$ & $8$ & ($-0.3$,$87.5$,$54.9$) & ($178.2$,$382.7$,$225.2$) & $-1.902$ & $0.621$ \\
 & & ($83.8$,$24.4$,$102.2$) & ($47.2$,$81.9$,$19.6$) & $0.019$ & $0.097$ \\
$DTG-25$ & $8$ & ($-5.0$,$92.5$,$16.6$) & ($278.6$,$813.6$,$187.2$) & $-1.686$ & $0.555$ \\
 & & ($81.0$,$5.1$,$93.2$) & ($26.1$,$46.4$,$22.2$) & $0.019$ & $0.023$ \\
$DTG-26$ & $8$ & ($101.7$,$-85.5$,$-6.5$) & ($405.3$,$-592.2$,$146.5$) & $-1.714$ & $0.695$ \\
 & & ($123.8$,$13.9$,$66.0$) & ($17.3$,$56.7$,$17.7$) & $0.021$ & $0.025$ \\
$DTG-27$ & $8$ & ($-34.7$,$15.2$,$-33.0$) & ($1482.5$,$140.2$,$37.8$) & $-1.419$ & $0.962$ \\
 & & ($282.3$,$14.3$,$28.4$) & ($140.8$,$102.0$,$15.3$) & $0.044$ & $0.018$ \\
$DTG-28$ & $7$ & ($54.0$,$23.8$,$21.5$) & ($754.8$,$178.0$,$268.5$) & $-1.604$ & $0.894$ \\
 & & ($152.4$,$13.5$,$115.8$) & ($52.0$,$165.8$,$19.3$) & $0.012$ & $0.047$ \\
$DTG-29$ & $7$ & ($-73.7$,$27.8$,$-59.6$) & ($453.0$,$168.9$,$145.6$) & $-1.840$ & $0.873$ \\
 & & ($97.4$,$13.1$,$31.3$) & ($22.8$,$79.7$,$13.5$) & $0.021$ & $0.049$ \\
$DTG-30$ & $7$ & ($1.0$,$225.1$,$-0.5$) & ($3.2$,$1885.4$,$0.7$) & $-1.566$ & $0.051$ \\
 & & ($15.4$,$4.1$,$4.0$) & ($2.4$,$5.9$,$0.5$) & $0.002$ & $0.016$ \\
$DTG-31$ & $7$ & ($-13.1$,$204.9$,$6.7$) & ($21.9$,$1671.3$,$3.0$) & $-1.622$ & $0.134$ \\
 & & ($14.2$,$3.2$,$10.1$) & ($3.4$,$14.6$,$2.5$) & $0.002$ & $0.008$ \\
$DTG-32$ & $7$ & ($-0.3$,$151.1$,$-0.6$) & ($129.6$,$1221.6$,$6.5$) & $-1.718$ & $0.358$ \\
 & & ($29.4$,$3.2$,$21.5$) & ($13.0$,$26.4$,$3.9$) & $0.007$ & $0.018$ \\
$DTG-33$ & $6$ & ($-77.4$,$-5.4$,$102.7$) & ($391.5$,$-37.0$,$277.8$) & $-1.839$ & $0.904$ \\
 & & ($7.4$,$15.6$,$44.2$) & ($27.8$,$91.4$,$23.2$) & $0.003$ & $0.048$ \\
$DTG-34$ & $6$ & ($-46.1$,$-89.0$,$-110.1$) & ($406.4$,$-779.5$,$336.6$) & $-1.584$ & $0.614$ \\
 & & ($122.1$,$22.8$,$90.4$) & ($40.1$,$147.0$,$39.6$) & $0.026$ & $0.046$ \\
$DTG-35$ & $6$ & ($30.7$,$94.9$,$76.6$) & ($249.9$,$523.2$,$128.5$) & $-1.845$ & $0.657$ \\
 & & ($104.6$,$13.4$,$22.0$) & ($60.1$,$128.2$,$6.5$) & $0.015$ & $0.116$ \\
$DTG-36$ & $6$ & ($94.4$,$-34.1$,$-5.9$) & ($696.9$,$-279.8$,$18.6$) & $-1.721$ & $0.881$ \\
 & & ($54.4$,$7.5$,$24.3$) & ($21.2$,$61.5$,$15.5$) & $0.018$ & $0.033$ \\
$DTG-37$ & $6$ & ($-92.8$,$3.4$,$-7.9$) & ($232.0$,$14.4$,$729.3$) & $-1.784$ & $0.594$ \\
 & & ($148.7$,$15.3$,$123.3$) & ($15.3$,$88.0$,$37.0$) & $0.019$ & $0.015$ \\
$DTG-38$ & $6$ & ($-8.6$,$264.0$,$-4.2$) & ($33.5$,$2207.0$,$1.8$) & $-1.470$ & $0.146$ \\
 & & ($19.1$,$7.5$,$10.4$) & ($6.2$,$10.7$,$1.2$) & $0.003$ & $0.014$ \\
\pagebreak
$DTG-39$ & $6$ & ($-57.0$,$-5.3$,$-10.4$) & ($304.3$,$-15.1$,$690.1$) & $-1.681$ & $0.668$ \\
 & & ($106.4$,$57.2$,$155.1$) & ($31.4$,$240.3$,$24.5$) & $0.012$ & $0.075$ \\
$DTG-40$ & $6$ & ($25.1$,$144.4$,$20.8$) & ($109.8$,$996.9$,$141.9$) & $-1.735$ & $0.357$ \\
 & & ($21.4$,$14.7$,$64.8$) & ($9.3$,$37.2$,$10.9$) & $0.010$ & $0.016$ \\
$DTG-41$ & $6$ & ($-94.1$,$40.1$,$59.5$) & ($634.7$,$344.4$,$157.2$) & $-1.663$ & $0.843$ \\
 & & ($81.2$,$9.4$,$53.7$) & ($42.1$,$63.8$,$18.7$) & $0.010$ & $0.029$ \\
$DTG-42$ & $6$ & ($18.0$,$16.3$,$6.6$) & ($1991.1$,$116.7$,$21.7$) & $-1.280$ & $0.977$ \\
 & & ($358.6$,$16.2$,$40.7$) & ($65.1$,$121.8$,$19.2$) & $0.016$ & $0.009$ \\
$DTG-43$ & $5$ & ($-31.7$,$27.9$,$0.9$) & ($528.6$,$187.6$,$26.4$) & $-1.859$ & $0.882$ \\
 & & ($83.7$,$8.1$,$32.2$) & ($25.8$,$61.0$,$7.9$) & $0.014$ & $0.040$ \\
$DTG-44$ & $5$ & ($50.6$,$108.2$,$-44.7$) & ($219.7$,$737.5$,$61.8$) & $-1.815$ & $0.530$ \\
 & & ($76.6$,$7.3$,$42.6$) & ($31.7$,$52.2$,$7.0$) & $0.024$ & $0.027$ \\
$DTG-45$ & $5$ & ($194.1$,$185.9$,$-29.8$) & ($618.0$,$1585.6$,$65.8$) & $-1.390$ & $0.596$ \\
 & & ($22.1$,$15.3$,$53.6$) & ($50.2$,$69.3$,$26.2$) & $0.024$ & $0.020$ \\
$DTG-46$ & $5$ & ($6.2$,$-17.1$,$-11.0$) & ($629.0$,$-146.2$,$18.9$) & $-1.821$ & $0.929$ \\
 & & ($104.1$,$12.6$,$18.2$) & ($25.3$,$84.5$,$7.0$) & $0.010$ & $0.023$ \\
$DTG-47$ & $5$ & ($16.3$,$230.8$,$0.3$) & ($4.1$,$1932.2$,$0.5$) & $-1.554$ & $0.053$ \\
 & & ($5.7$,$5.6$,$6.1$) & ($1.3$,$10.3$,$0.3$) & $0.003$ & $0.010$ \\
$DTG-48$ & $5$ & ($-2.5$,$244.5$,$-6.3$) & ($4.0$,$2039.1$,$1.0$) & $-1.524$ & $0.052$ \\
 & & ($4.1$,$1.4$,$3.2$) & ($0.6$,$10.1$,$0.1$) & $0.003$ & $0.004$ \\
$DTG-49$ & $5$ & ($104.9$,$150.8$,$4.1$) & ($274.6$,$1299.9$,$14.8$) & $-1.612$ & $0.477$ \\
 & & ($77.6$,$17.7$,$22.3$) & ($10.4$,$49.1$,$11.9$) & $0.013$ & $0.012$ \\
$DTG-50$ & $5$ & ($-67.2$,$-78.5$,$-29.5$) & ($270.9$,$-464.8$,$109.2$) & $-1.859$ & $0.666$ \\
 & & ($61.4$,$17.6$,$45.7$) & ($7.6$,$113.2$,$16.4$) & $0.023$ & $0.051$ \\
$DTG-51$ & $5$ & ($48.4$,$-136.4$,$-25.7$) & ($247.9$,$-1011.5$,$48.9$) & $-1.725$ & $0.494$ \\
 & & ($133.9$,$20.8$,$28.2$) & ($38.0$,$41.4$,$16.3$) & $0.027$ & $0.039$ \\
$DTG-52$ & $5$ & ($151.1$,$181.8$,$-83.0$) & ($440.9$,$1352.3$,$737.1$) & $-1.357$ & $0.498$ \\
 & & ($13.1$,$62.5$,$171.2$) & ($46.9$,$119.8$,$29.6$) & $0.035$ & $0.025$ \\
\enddata
\end{deluxetable*}


==> Tables/cluster_stellar_results_table.tex <==
\startlongtable
\begin{deluxetable*}{l  c  c  c  c}
\tablecaption{DTGs Identified by \HDBSCAN \label{tab:cluster_results}}
\tablehead{\colhead{Star Name} & \colhead{[Fe/H]} & \colhead{[C/Fe]} & \colhead{[C/Fe]$_{c}$} & \colhead{[$\alpha$/Fe]}}
\startdata
\multicolumn{5}{c}{$DTG-1$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J035806.92$-$412551.4 & $-1.061$ & $\dots$ & $\dots$ & $\dots$ \\
J060951.09$-$233050.3 & $-0.816$ & $\dots$ & $\dots$ & $\dots$ \\
J062203.79$-$215529.0 & $-1.034$ & $+0.094$ & $+0.094$ & $\dots$ \\
J075523.99$+$352005.5 & $-0.927$ & $-0.273$ & $-0.273$ & $+0.018$ \\
J095327.59$-$271710.2 & $-1.430$ & $\dots$ & $\dots$ & $\dots$ \\
J102813.29$-$294653.2 & $-1.231$ & $\dots$ & $\dots$ & $\dots$ \\
J114658.41$+$483515.4 & $-1.172$ & $-0.340$ & $-0.340$ & $-0.029$ \\
J115951.48$-$390527.5 & $-1.041$ & $+0.077$ & $+0.077$ & $+0.167$ \\
J133023.82$-$000654.8 & $-0.878$ & $\dots$ & $\dots$ & $\dots$ \\
J155713.55$-$375241.2 & $-1.169$ & $-0.216$ & $-0.186$ & $\dots$ \\
J160749.07$+$142013.2 & $-1.468$ & $-0.208$ & $-0.208$ & $-0.007$ \\
J161730.55$-$193225.6 & $-1.094$ & $+0.402$ & $+0.422$ & $-0.035$ \\
J173313.27$-$610148.2 & $-1.359$ & $-0.207$ & $-0.207$ & $\dots$ \\
J173346.78$-$674403.0 & $-1.658$ & $\dots$ & $\dots$ & $\dots$ \\
J183718.56$-$641756.9 & $-0.871$ & $\dots$ & $\dots$ & $\dots$ \\
J195013.73$-$771450.7 & $-1.102$ & $-0.558$ & $-0.558$ & $-0.275$ \\
J202034.71$-$275711.3 & $-1.083$ & $-0.143$ & $-0.143$ & $+0.049$ \\
J205902.49$+$184702.0 & $-1.382$ & $-0.268$ & $-0.258$ & $\dots$ \\
J220339.84$-$644528.9 & $-0.872$ & $\dots$ & $\dots$ & $\dots$ \\
J222900.16$-$173756.1 & $-1.108$ & $\dots$ & $\dots$ & $\dots$ \\
J223557.26$-$243411.6 & $-0.945$ & $-0.265$ & $-0.265$ & $+0.062$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.105\pm0.222$ & $-0.225\pm0.169$ & $-0.219\pm0.170$ & $+0.018\pm0.086$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-2$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: GL-1: \citet{Li2019}} \\
\multicolumn{5}{c}{Group Assoc: CDTG-6: \citet{Gudin2021}} \\
\multicolumn{5}{c}{Stellar Assoc: 2MASS J06290787-6709523 (CDTG-8: \citet{Gudin2021})} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J000212.23$-$224138.9 & $-2.369$ & $+0.585$ & $+0.595$ & $+0.106$ \\
J013043.37$-$545515.1 & $-2.539$ & $+0.567$ & $+0.597$ & $+0.455$ \\
J013152.15$-$654754.8 & $-0.961$ & $+0.107$ & $+0.107$ & $+0.246$ \\
J042139.28$-$570515.3 & $-1.730$ & $\dots$ & $\dots$ & $\dots$ \\
J062907.88$-$670952.2 & $-2.856$ & $+0.056$ & $+0.716$ & $+0.382$ \\
J110822.39$-$161013.4 & $-1.840$ & $\dots$ & $\dots$ & $\dots$ \\
J124700.20$-$701645.9 & $-1.652$ & $+0.049$ & $+0.109$ & $+0.087$ \\
J131609.95$-$481722.4 & $-2.274$ & $+0.199$ & $+0.249$ & $+0.501$ \\
J140129.33$+$112636.0 & $-2.206$ & $-0.537$ & $+0.123$ & $+0.378$ \\
J162811.79$-$015518.9 & $-1.560$ & $\dots$ & $\dots$ & $\dots$ \\
J190807.44$-$785039.9 & $-2.410$ & $+0.121$ & $+0.621$ & $+0.384$ \\
J193222.62$-$752849.4 & $-2.578$ & $+0.164$ & $+0.174$ & $+0.353$ \\
J195332.63$-$752513.5 & $-1.604$ & $-0.259$ & $-0.009$ & $+0.462$ \\
J200528.77$-$543126.0 & $-2.941$ & $+0.817$ & $+0.837$ & $+0.354$ \\
J201948.67$-$240304.0 & $-1.790$ & $\dots$ & $\dots$ & $\dots$ \\
J211726.95$+$135951.4 & $-2.680$ & $+0.363$ & $+0.383$ & $+0.197$ \\
J214538.50$+$235111.4 & $-2.505$ & $+0.314$ & $+0.384$ & $+0.330$ \\
J223002.39$-$633219.1 & $-2.354$ & $-0.599$ & $+0.161$ & $\dots$ \\
J230352.75$-$311241.7 & $-1.623$ & $+0.258$ & $+0.278$ & $+0.565$ \\
J234425.11$-$405834.1 & $-1.583$ & $+0.175$ & $+0.195$ & $+0.237$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.132\pm0.544$ & $+0.200\pm0.355$ & $+0.301\pm0.267$ & $+0.342\pm0.138$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-3$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J005231.11$+$375828.3 & $-2.230$ & $+0.810$ & $+0.820$ & $+0.403$ \\
J034206.57$+$014250.6 & $-1.730$ & $\dots$ & $\dots$ & $\dots$ \\
J050218.98$-$515205.4 & $-1.735$ & $+0.294$ & $+0.314$ & $+0.217$ \\
J055056.57$-$200841.8 & $-1.994$ & $+0.381$ & $+0.391$ & $+0.089$ \\
J060322.01$-$354619.4 & $-1.570$ & $\dots$ & $\dots$ & $\dots$ \\
J060600.02$-$690742.4 & $-2.150$ & $-0.064$ & $+0.226$ & $+0.217$ \\
J072030.82$-$624045.1 & $-2.025$ & $-0.371$ & $+0.149$ & $+0.289$ \\
J091848.48$+$071336.0 & $-2.071$ & $-0.161$ & $-0.011$ & $+0.497$ \\
J092703.01$+$420449.3 & $-1.920$ & $-0.075$ & $+0.045$ & $+0.440$ \\
J093331.85$-$013038.3 & $-1.660$ & $\dots$ & $\dots$ & $\dots$ \\
J104608.76$-$115025.0 & $-1.540$ & $\dots$ & $\dots$ & $\dots$ \\
J115153.40$+$815115.1 & $-2.094$ & $-0.146$ & $-0.096$ & $+0.155$ \\
J142616.56$+$810245.0 & $-2.539$ & $-0.226$ & $+0.504$ & $+0.409$ \\
J150901.99$-$215246.9 & $-1.480$ & $\dots$ & $\dots$ & $\dots$ \\
J174931.90$-$531427.4 & $-1.886$ & $+0.471$ & $+0.481$ & $+0.350$ \\
J182534.41$+$473329.6 & $-1.884$ & $+0.003$ & $+0.183$ & $+0.257$ \\
J201211.38$-$561617.8 & $-2.152$ & $-0.061$ & $+0.559$ & $\dots$ \\
J232540.59$+$211547.6 & $-1.940$ & $+0.242$ & $+0.252$ & $+0.224$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.919\pm0.268$ & $-0.006\pm0.331$ & $+0.280\pm0.251$ & $+0.291\pm0.126$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-4$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: J060903.60-712226.0 (Sausage: \citet{Cordoni2021})} \\
\multicolumn{5}{c}{Stellar Assoc: 2MASS J06090353-7122260 (CDTG-14: \citet{Gudin2021})} \\
\multicolumn{5}{c}{Stellar Assoc: CS29512-51 (DTG-13: \citet{Limberg2021a})} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J022635.59$-$611822.9 & $-2.375$ & $-0.315$ & $+0.285$ & $+0.112$ \\
J053322.44$-$503025.8 & $-2.309$ & $+0.408$ & $+0.648$ & $+0.276$ \\
J060903.58$-$712225.9 & $-2.842$ & $+0.805$ & $+1.035$ & $+0.252$ \\
J113738.01$-$520224.8 & $-2.494$ & $+0.805$ & $+1.015$ & $-0.198$ \\
J145619.30$+$082949.0 & $-2.487$ & $-0.180$ & $+0.360$ & $+0.457$ \\
J150204.34$+$113159.4 & $-2.339$ & $+0.054$ & $+0.274$ & $+0.310$ \\
J160911.64$+$300842.4 & $-2.282$ & $-0.405$ & $+0.285$ & $+0.534$ \\
J163136.12$-$012341.1 & $-2.190$ & $\dots$ & $\dots$ & $\dots$ \\
J163504.81$+$113719.2 & $-2.669$ & $-0.373$ & $+0.367$ & $+0.363$ \\
J170247.80$+$255912.9 & $-2.504$ & $-0.059$ & $+0.551$ & $+0.343$ \\
J200605.29$-$431513.6 & $-3.170$ & $\dots$ & $\dots$ & $\dots$ \\
J203759.27$-$605642.1 & $-2.620$ & $\dots$ & $\dots$ & $\dots$ \\
J205236.27$-$524103.4 & $-2.313$ & $+0.057$ & $+0.587$ & $+0.314$ \\
J212541.31$-$542811.2 & $-2.540$ & $\dots$ & $\dots$ & $\dots$ \\
J212951.05$-$542808.4 & $-2.150$ & $\dots$ & $\dots$ & $\dots$ \\
J222025.81$-$102320.2 & $-2.614$ & $+0.648$ & $+0.658$ & $+0.482$ \\
J225118.77$-$381438.6 & $-2.088$ & $+0.437$ & $+0.447$ & $+0.378$ \\
J230932.09$-$713250.7 & $-2.384$ & $-0.564$ & $+0.016$ & $+0.051$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.425\pm0.233$ & $+0.085\pm0.479$ & $+0.464\pm0.286$ & $+0.332\pm0.162$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-5$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: CDTG-22: \citet{Gudin2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J012423.81$-$324914.9 & $-1.740$ & $\dots$ & $\dots$ & $\dots$ \\
J013722.46$-$461111.3 & $-1.419$ & $-0.276$ & $-0.096$ & $+0.020$ \\
J025336.14$-$623451.1 & $-1.783$ & $+0.185$ & $+0.205$ & $+0.208$ \\
J030605.97$-$525143.2 & $-2.097$ & $+0.530$ & $+0.540$ & $+0.101$ \\
J040822.08$-$805405.5 & $-2.178$ & $+0.067$ & $+0.407$ & $+0.128$ \\
J042427.25$-$815749.3 & $-2.203$ & $+0.289$ & $+0.299$ & $\dots$ \\
J063641.43$-$693137.7 & $-2.220$ & $\dots$ & $\dots$ & $\dots$ \\
J103509.86$-$141628.4 & $-2.306$ & $+0.768$ & $+0.778$ & $+0.169$ \\
J121129.42$-$413317.2 & $-0.870$ & $\dots$ & $\dots$ & $\dots$ \\
J121816.89$-$380507.9 & $-1.940$ & $\dots$ & $\dots$ & $\dots$ \\
J142038.84$-$842819.9 & $-1.828$ & $+0.112$ & $+0.332$ & $+0.348$ \\
J162722.50$-$084836.3 & $-2.713$ & $+0.208$ & $+0.778$ & $+0.459$ \\
J171848.67$-$832249.8 & $-2.110$ & $\dots$ & $\dots$ & $\dots$ \\
J182116.00$-$365755.4 & $-2.466$ & $+0.134$ & $+0.634$ & $+0.707$ \\
J185239.81$+$412928.8 & $-1.769$ & $+0.052$ & $+0.142$ & $+0.757$ \\
J211902.73$+$331846.0 & $-2.105$ & $-0.175$ & $+0.025$ & $+0.255$ \\
J233624.25$-$470759.8 & $-1.870$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.049\pm0.368$ & $+0.131\pm0.256$ & $+0.360\pm0.296$ & $+0.248\pm0.248$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-6$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: J053431.31+035228.4 (DTG-35: \citet{Yuan2020b})} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J022058.73$-$670804.4 & $-2.518$ & $-0.202$ & $+0.398$ & $-0.118$ \\
J033913.71$+$031034.4 & $-2.311$ & $+0.185$ & $+0.455$ & $+0.461$ \\
J035518.72$-$354055.4 & $-2.256$ & $+1.012$ & $+1.072$ & $+0.306$ \\
J053431.31$+$035228.4 & $-2.496$ & $+0.566$ & $+0.576$ & $\dots$ \\
J082030.56$-$615527.6 & $-2.312$ & $+0.003$ & $+0.223$ & $+0.202$ \\
J094744.93$-$704553.3 & $-2.204$ & $+0.134$ & $+0.334$ & $-0.170$ \\
J094918.88$+$320106.0 & $-2.294$ & $-0.240$ & $+0.490$ & $+0.413$ \\
J104530.03$-$195540.3 & $-1.840$ & $\dots$ & $\dots$ & $\dots$ \\
J123409.62$-$345344.0 & $-2.418$ & $-0.121$ & $+0.579$ & $-0.033$ \\
J132841.04$-$011109.1 & $-2.440$ & $\dots$ & $\dots$ & $\dots$ \\
J152101.40$+$781607.6 & $-3.541$ & $+0.527$ & $+0.677$ & $\dots$ \\
J194339.30$+$774900.4 & $-2.714$ & $-0.127$ & $+0.533$ & $+0.282$ \\
J202221.56$-$121443.9 & $-2.540$ & $\dots$ & $\dots$ & $\dots$ \\
J210308.37$-$491640.6 & $-2.283$ & $-0.125$ & $+0.555$ & $\dots$ \\
J211353.40$-$680637.1 & $-2.300$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.358\pm0.194$ & $+0.020\pm0.358$ & $+0.506\pm0.162$ & $+0.184\pm0.249$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-7$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Comoving: \citet{Myeong2017}} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Monty2020}} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J013855.36$-$522631.5 & $-2.020$ & $\dots$ & $\dots$ & $\dots$ \\
J020227.66$-$592039.4 & $-1.930$ & $+0.403$ & $+0.413$ & $+0.324$ \\
J031038.90$-$471725.4 & $-1.989$ & $+0.025$ & $+0.305$ & $+0.064$ \\
J041642.57$-$421600.0 & $-1.720$ & $\dots$ & $\dots$ & $\dots$ \\
J065250.96$+$244025.9 & $-1.927$ & $-0.047$ & $+0.383$ & $+0.531$ \\
J082806.59$-$784217.1 & $-2.260$ & $\dots$ & $\dots$ & $\dots$ \\
J111208.32$-$044840.0 & $-2.050$ & $\dots$ & $\dots$ & $\dots$ \\
J113720.03$+$184530.8 & $-2.575$ & $-0.514$ & $-0.124$ & $+0.534$ \\
J162202.39$+$070037.9 & $-2.399$ & $+0.036$ & $+0.576$ & $+0.463$ \\
J180757.82$-$795618.2 & $-2.379$ & $-0.148$ & $+0.492$ & $+0.430$ \\
J182721.67$-$493711.2 & $-1.620$ & $\dots$ & $\dots$ & $\dots$ \\
J191200.66$-$630256.2 & $-1.636$ & $-0.246$ & $-0.026$ & $+0.092$ \\
J201236.69$-$575704.5 & $-2.211$ & $+0.213$ & $+0.723$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.047\pm0.300$ & $-0.025\pm0.269$ & $+0.396\pm0.289$ & $+0.395\pm0.204$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-8$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Comoving: \citet{Myeong2017}} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Monty2020}} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J010651.90$-$524410.5 & $-3.269$ & $+0.195$ & $+0.205$ & $+0.218$ \\
J023240.42$-$370811.0 & $-2.620$ & $\dots$ & $\dots$ & $\dots$ \\
J033515.22$+$782325.2 & $-2.414$ & $-0.360$ & $+0.400$ & $+0.402$ \\
J042253.10$-$652231.3 & $-2.780$ & $\dots$ & $\dots$ & $\dots$ \\
J043133.35$-$733716.8 & $-1.860$ & $+0.464$ & $+0.474$ & $+0.321$ \\
J065541.43$-$431358.0 & $-2.354$ & $-0.238$ & $+0.472$ & $+0.344$ \\
J113457.92$+$003512.2 & $-1.940$ & $\dots$ & $\dots$ & $\dots$ \\
J132400.06$-$174810.1 & $-1.975$ & $+0.365$ & $+0.435$ & $+0.139$ \\
J143359.19$-$832827.2 & $-1.870$ & $\dots$ & $\dots$ & $\dots$ \\
J174732.57$-$562508.0 & $-1.590$ & $\dots$ & $\dots$ & $\dots$ \\
J221124.59$-$375310.2 & $-2.146$ & $-0.502$ & $+0.208$ & $+0.223$ \\
J230353.29$-$413948.2 & $-1.942$ & $-0.172$ & $-0.012$ & $-0.203$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.117\pm0.456$ & $-0.057\pm0.386$ & $+0.383\pm0.182$ & $+0.252\pm0.169$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-9$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: 5921375409886676224 (NGC~6397: \citet{Vasiliev2021})} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J162832.99$+$172232.8 & $-2.570$ & $-0.383$ & $+0.347$ & $+0.398$ \\
J164024.68$+$155040.7 & $-2.895$ & $-0.601$ & $+0.069$ & $+0.521$ \\
J170132.06$-$550745.7 & $-2.190$ & $+0.435$ & $+0.445$ & $-0.068$ \\
J173857.10$-$535540.9 & $-2.480$ & $\dots$ & $\dots$ & $\dots$ \\
J173930.96$-$533458.8 & $-2.347$ & $+0.431$ & $+0.481$ & $+0.285$ \\
J173959.93$-$533519.3 & $-2.330$ & $\dots$ & $\dots$ & $\dots$ \\
J174010.59$-$535957.6 & $-2.730$ & $\dots$ & $\dots$ & $\dots$ \\
J174049.22$-$532629.9 & $-2.296$ & $+0.513$ & $+0.863$ & $\dots$ \\
J174145.11$-$533142.3 & $-2.390$ & $\dots$ & $\dots$ & $\dots$ \\
J174351.13$-$535933.4 & $-2.499$ & $-0.339$ & $+0.231$ & $+0.191$ \\
J202753.01$-$514113.7 & $-2.684$ & $-0.077$ & $+0.633$ & $+0.164$ \\
J205453.08$-$471029.0 & $-2.562$ & $-0.252$ & $+0.468$ & $+0.121$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.489\pm0.200$ & $-0.064\pm0.448$ & $+0.440\pm0.233$ & $+0.214\pm0.195$\\
\multicolumn{5}{c}{$DTG-10$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Group Assoc: DTG-23: \citet{Limberg2021a}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J004251.85$+$192535.9 & $-1.561$ & $+0.100$ & $+0.120$ & $+0.361$ \\
J010030.72$+$041545.2 & $-1.634$ & $+0.081$ & $+0.101$ & $+0.197$ \\
J033215.69$-$064429.7 & $-2.096$ & $+0.131$ & $+0.481$ & $+0.460$ \\
J042515.21$-$621320.9 & $-2.378$ & $+0.175$ & $+0.605$ & $+0.024$ \\
J052903.45$-$610544.6 & $-2.630$ & $\dots$ & $\dots$ & $\dots$ \\
J060120.29$-$014744.4 & $-1.742$ & $+0.051$ & $+0.071$ & $+0.307$ \\
J074503.51$+$095614.8 & $-2.638$ & $-0.485$ & $+0.255$ & $+0.339$ \\
J100112.02$-$295847.7 & $-2.167$ & $-0.333$ & $+0.327$ & $+0.527$ \\
J152604.25$+$460802.8 & $-2.094$ & $-0.054$ & $+0.136$ & $+0.314$ \\
J192020.70$-$662720.4 & $-2.298$ & $+0.075$ & $+0.715$ & $\dots$ \\
J202649.50$-$473428.1 & $-2.220$ & $\dots$ & $\dots$ & $\dots$ \\
J211151.21$-$525707.8 & $-1.407$ & $+0.284$ & $+0.304$ & $+0.290$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.089\pm0.408$ & $+0.097\pm0.159$ & $+0.294\pm0.220$ & $+0.326\pm0.133$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-11$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Comoving: \citet{Myeong2017}} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: Ryu~879~(RLGC~2): \citet{Vasiliev2021}} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J140702.07$+$141218.9 & $-2.421$ & $-0.168$ & $+0.432$ & $\dots$ \\
J142958.40$+$450202.5 & $-2.004$ & $+0.121$ & $+0.441$ & $+0.497$ \\
J155358.31$+$433328.1 & $-1.573$ & $-0.508$ & $+0.012$ & $+0.159$ \\
J172609.07$-$673207.9 & $-1.870$ & $\dots$ & $\dots$ & $\dots$ \\
J175103.69$-$564506.6 & $-2.015$ & $-0.411$ & $+0.259$ & $\dots$ \\
J183838.49$-$704134.1 & $-2.280$ & $\dots$ & $\dots$ & $\dots$ \\
J184403.71$-$485458.3 & $-2.580$ & $\dots$ & $\dots$ & $\dots$ \\
J202440.09$-$223954.8 & $-1.870$ & $\dots$ & $\dots$ & $\dots$ \\
J203725.57$-$231906.2 & $-2.230$ & $\dots$ & $\dots$ & $\dots$ \\
J212631.80$+$203147.0 & $-3.041$ & $-0.190$ & $+0.540$ & $+0.453$ \\
J221208.15$-$421521.0 & $-1.971$ & $+0.208$ & $+0.218$ & $+0.066$ \\
J234115.83$-$640644.1 & $-2.810$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.166\pm0.427$ & $-0.162\pm0.267$ & $+0.336\pm0.186$ & $+0.296\pm0.196$\\
\multicolumn{5}{c}{$DTG-12$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: 2MASS J18082002-5104378 (P: \citet{Sestito2019})} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J053600.74$-$495152.9 & $-0.980$ & $\dots$ & $\dots$ & $\dots$ \\
J054854.25$-$400434.9 & $-1.240$ & $\dots$ & $\dots$ & $\dots$ \\
J092611.51$+$003113.1 & $-1.514$ & $\dots$ & $\dots$ & $\dots$ \\
J130915.78$+$464059.3 & $-0.970$ & $-0.017$ & $-0.017$ & $+0.393$ \\
J131612.23$-$141749.9 & $-0.879$ & $\dots$ & $\dots$ & $\dots$ \\
J142002.95$+$593628.5 & $-1.162$ & $-0.430$ & $-0.430$ & $+0.287$ \\
J144530.96$-$021408.1 & $-0.927$ & $+0.365$ & $+0.365$ & $+0.530$ \\
J163748.45$+$073437.1 & $-0.887$ & $+0.237$ & $+0.237$ & $+0.548$ \\
J172546.59$-$851301.3 & $-1.058$ & $+0.251$ & $+0.251$ & $+0.391$ \\
J180820.02$-$510437.9 & $-3.080$ & $\dots$ & $\dots$ & $\dots$ \\
J185441.76$-$480638.2 & $-1.540$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.085\pm0.252$ & $+0.209\pm0.276$ & $+0.209\pm0.276$ & $+0.427\pm0.107$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-13$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J030523.26$+$284349.2 & $-1.390$ & $-0.298$ & $-0.298$ & $+0.115$ \\
J031017.10$+$485637.5 & $-0.847$ & $-0.328$ & $-0.328$ & $-0.018$ \\
J032236.53$+$085938.3 & $-1.092$ & $-0.261$ & $-0.261$ & $+0.037$ \\
J042126.40$-$052315.1 & $-0.833$ & $\dots$ & $\dots$ & $\dots$ \\
J044336.26$+$393610.6 & $-1.175$ & $+0.137$ & $+0.147$ & $+0.116$ \\
J055949.46$-$304800.6 & $-0.935$ & $\dots$ & $\dots$ & $\dots$ \\
J060747.14$-$372449.9 & $-1.207$ & $\dots$ & $\dots$ & $\dots$ \\
J070251.09$+$050147.8 & $-2.485$ & $+0.728$ & $+1.198$ & $\dots$ \\
J102956.59$-$403509.1 & $-1.333$ & $\dots$ & $\dots$ & $\dots$ \\
J164308.55$+$042600.6 & $-0.992$ & $+0.013$ & $+0.013$ & $+0.124$ \\
J230003.92$-$745124.3 & $-0.820$ & $-0.368$ & $-0.368$ & $+0.026$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.063\pm0.292$ & $-0.235\pm0.221$ & $-0.236\pm0.223$ & $+0.070\pm0.058$\\
\multicolumn{5}{c}{$DTG-14$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J140153.46$-$342727.3 & $-1.788$ & $-0.086$ & $+0.054$ & $+0.216$ \\
J160226.98$-$220056.9 & $-1.910$ & $\dots$ & $\dots$ & $\dots$ \\
J161504.74$-$164053.1 & $-1.330$ & $\dots$ & $\dots$ & $\dots$ \\
J161926.58$-$100956.5 & $-1.710$ & $\dots$ & $\dots$ & $\dots$ \\
J171319.75$-$711301.1 & $-2.617$ & $-0.041$ & $+0.659$ & $\dots$ \\
J174257.89$+$041738.1 & $-2.747$ & $+0.007$ & $+0.237$ & $+0.332$ \\
J175808.77$-$501702.5 & $-1.979$ & $-0.127$ & $+0.243$ & $+0.435$ \\
J182720.15$-$484515.6 & $-1.630$ & $\dots$ & $\dots$ & $\dots$ \\
J200828.34$+$101158.2 & $-2.515$ & $-0.254$ & $+0.476$ & $+0.440$ \\
J202436.59$-$172705.6 & $-2.280$ & $\dots$ & $\dots$ & $\dots$ \\
J211143.61$-$083626.3 & $-2.445$ & $+0.123$ & $+0.453$ & $+0.468$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.069\pm0.476$ & $-0.062\pm0.123$ & $+0.351\pm0.214$ & $+0.430\pm0.087$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-15$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J161808.26$-$170826.0 & $-1.340$ & $\dots$ & $\dots$ & $\dots$ \\
J170707.57$-$781756.2 & $-2.711$ & $+0.059$ & $+0.069$ & $\dots$ \\
J170737.82$-$622222.6 & $-1.400$ & $\dots$ & $\dots$ & $\dots$ \\
J171511.94$-$163643.4 & $-2.070$ & $\dots$ & $\dots$ & $\dots$ \\
J175059.61$+$184510.9 & $-1.977$ & $-0.206$ & $+0.174$ & $+0.324$ \\
J180626.25$-$564112.8 & $-2.220$ & $+0.286$ & $+0.726$ & $+0.587$ \\
J181312.89$+$174849.4 & $-1.988$ & $-0.472$ & $+0.058$ & $+0.361$ \\
J183033.24$-$643050.9 & $-1.750$ & $\dots$ & $\dots$ & $\dots$ \\
J183120.01$-$512743.9 & $-2.310$ & $\dots$ & $\dots$ & $\dots$ \\
J202217.63$-$555640.7 & $-2.040$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.995\pm0.402$ & $-0.080\pm0.298$ & $+0.101\pm0.068$ & $+0.343\pm0.106$\\
\multicolumn{5}{c}{$DTG-16$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J133308.90$-$465407.9 & $-2.936$ & $+0.025$ & $+0.405$ & $\dots$ \\
J140605.13$-$773910.8 & $-2.050$ & $\dots$ & $\dots$ & $\dots$ \\
J142745.95$-$485909.0 & $-2.100$ & $\dots$ & $\dots$ & $\dots$ \\
J160852.85$-$211043.8 & $-1.356$ & $-0.221$ & $-0.201$ & $+0.080$ \\
J162905.39$-$134850.1 & $-1.660$ & $\dots$ & $\dots$ & $\dots$ \\
J164239.34$-$830636.6 & $-2.357$ & $+0.693$ & $+0.763$ & $+0.186$ \\
J165837.21$+$015343.0 & $-2.620$ & $+0.520$ & $+0.530$ & $+0.452$ \\
J182504.27$-$420839.6 & $-1.530$ & $\dots$ & $\dots$ & $\dots$ \\
J195343.57$+$120836.9 & $-2.126$ & $-0.025$ & $+0.185$ & $+0.057$ \\
J195739.81$-$782513.9 & $-1.830$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.046\pm0.484$ & $+0.146\pm0.407$ & $+0.370\pm0.346$ & $+0.120\pm0.153$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-17$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J055446.91$-$830119.8 & $-2.204$ & $-0.147$ & $+0.333$ & $+0.501$ \\
J125523.76$-$842816.3 & $-2.690$ & $+0.429$ & $+0.749$ & $+0.093$ \\
J132736.76$-$171038.5 & $-2.415$ & $-0.486$ & $-0.136$ & $\dots$ \\
J133609.38$-$440853.8 & $-2.189$ & $+0.232$ & $+0.522$ & $+0.198$ \\
J165243.13$-$671952.2 & $-3.178$ & $+0.827$ & $+0.837$ & $\dots$ \\
J200659.85$-$784041.2 & $-2.000$ & $\dots$ & $\dots$ & $\dots$ \\
J201854.85$-$142852.3 & $-1.941$ & $-0.156$ & $+0.104$ & $+0.422$ \\
J212237.23$-$700623.1 & $-1.250$ & $\dots$ & $\dots$ & $\dots$ \\
J221153.49$-$120918.3 & $-2.278$ & $-0.374$ & $+0.156$ & $+0.193$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.227\pm0.478$ & $-0.009\pm0.480$ & $+0.357\pm0.355$ & $+0.255\pm0.183$\\
\multicolumn{5}{c}{$DTG-18$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Group Assoc: CDTG-13: \citet{Gudin2021}} \\
\multicolumn{5}{c}{Group Assoc: DTG-30: \citet{Limberg2021a}} \\
\multicolumn{5}{c}{Stellar Assoc: 2MASS J18562774-7251331 (CDTG-13: \citet{Gudin2021})} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J002755.10$+$345806.7 & $-2.126$ & $-0.333$ & $+0.147$ & $+0.429$ \\
J075113.42$-$593835.4 & $-1.460$ & $\dots$ & $\dots$ & $\dots$ \\
J094804.26$-$714248.8 & $-2.120$ & $\dots$ & $\dots$ & $\dots$ \\
J103948.94$+$345928.5 & $-2.548$ & $-0.367$ & $+0.243$ & $+0.485$ \\
J170419.78$+$632522.4 & $-2.153$ & $-0.426$ & $+0.284$ & $+0.444$ \\
J183958.04$+$482033.7 & $-2.442$ & $-0.476$ & $+0.184$ & $+0.373$ \\
J185627.75$-$725133.0 & $-2.640$ & $-0.348$ & $+0.402$ & $\dots$ \\
J191058.03$-$854037.1 & $-1.933$ & $-0.366$ & $+0.204$ & $+0.442$ \\
J234949.65$-$794848.3 & $-1.751$ & $-0.116$ & $-0.096$ & $+0.081$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.137\pm0.370$ & $-0.376\pm0.068$ & $+0.224\pm0.129$ & $+0.436\pm0.040$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-19$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J012730.06$-$662202.7 & $-0.981$ & $\dots$ & $\dots$ & $\dots$ \\
J103914.94$+$734827.9 & $-1.034$ & $+0.253$ & $+0.253$ & $+0.361$ \\
J104303.65$-$064303.8 & $-1.335$ & $+0.146$ & $+0.146$ & $+0.478$ \\
J110536.78$-$053953.0 & $-0.836$ & $\dots$ & $\dots$ & $\dots$ \\
J120210.52$-$755259.1 & $-1.348$ & $\dots$ & $\dots$ & $\dots$ \\
J181458.98$+$585256.5 & $-0.818$ & $+0.172$ & $+0.172$ & $+0.294$ \\
J202332.04$-$172322.6 & $-1.491$ & $\dots$ & $\dots$ & $\dots$ \\
J210247.49$-$471433.2 & $-0.872$ & $\dots$ & $\dots$ & $\dots$ \\
J222616.58$-$664225.8 & $-1.010$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.054\pm0.251$ & $+0.180\pm0.051$ & $+0.180\pm0.051$ & $+0.373\pm0.081$\\
\multicolumn{5}{c}{$DTG-20$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J054409.33$-$382015.0 & $-1.410$ & $+0.300$ & $+0.320$ & $+0.459$ \\
J074500.53$-$692309.1 & $-2.004$ & $+0.096$ & $+0.106$ & $-0.039$ \\
J082238.66$-$673333.3 & $-1.560$ & $\dots$ & $\dots$ & $\dots$ \\
J090305.04$-$204741.4 & $-1.595$ & $-0.176$ & $+0.074$ & $-0.101$ \\
J093436.49$+$103602.5 & $-2.245$ & $+0.568$ & $+0.578$ & $+0.630$ \\
J134338.66$+$484426.2 & $-3.145$ & $+1.137$ & $+1.137$ & $+0.042$ \\
J180234.56$-$610816.1 & $-1.764$ & $+0.329$ & $+0.349$ & $+0.430$ \\
J215816.38$+$394610.5 & $-1.772$ & $+0.103$ & $+0.123$ & $+0.309$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.754\pm0.380$ & $+0.263\pm0.382$ & $+0.310\pm0.326$ & $+0.254\pm0.277$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-21$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J150528.98$-$222309.3 & $-2.160$ & $\dots$ & $\dots$ & $\dots$ \\
J161021.11$+$002326.3 & $-2.004$ & $-0.187$ & $+0.213$ & $+0.587$ \\
J161425.47$-$004504.6 & $-2.071$ & $-0.149$ & $+0.421$ & $\dots$ \\
J183424.80$-$641039.7 & $-2.830$ & $\dots$ & $\dots$ & $\dots$ \\
J183617.59$-$525851.6 & $-2.059$ & $+0.325$ & $+0.615$ & $\dots$ \\
J190149.51$-$484436.0 & $-2.001$ & $+0.046$ & $+0.446$ & $\dots$ \\
J194600.15$-$484420.3 & $-1.372$ & $-0.550$ & $-0.390$ & $-0.122$ \\
J195345.83$-$530552.0 & $-1.679$ & $+0.116$ & $+0.456$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.037\pm0.180$ & $-0.043\pm0.291$ & $+0.435\pm0.166$ & $+0.232\pm0.373$\\
\multicolumn{5}{c}{$DTG-22$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: DTG-30: \citet{Limberg2021a}} \\
\multicolumn{5}{c}{Stellar Assoc: 2MASS J10492192-1154173 (CDTG-1: \citet{Gudin2021})} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J055023.17$-$613652.7 & $-2.521$ & $+0.068$ & $+0.288$ & $+0.368$ \\
J104921.90$-$115417.4 & $-1.990$ & $\dots$ & $\dots$ & $\dots$ \\
J165147.71$+$384428.7 & $-2.311$ & $+0.277$ & $+0.287$ & $+0.028$ \\
J171639.42$-$871123.8 & $-2.383$ & $+0.826$ & $+0.836$ & $+0.161$ \\
J181948.24$-$531056.4 & $-2.236$ & $+0.489$ & $+0.549$ & $+0.194$ \\
J201252.88$+$012418.3 & $-2.246$ & $-0.308$ & $+0.392$ & $+0.544$ \\
J204355.75$-$563629.2 & $-1.950$ & $\dots$ & $\dots$ & $\dots$ \\
J235053.48$+$114234.8 & $-2.053$ & $-0.047$ & $+0.113$ & $+0.534$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.215\pm0.197$ & $+0.198\pm0.388$ & $+0.363\pm0.237$ & $+0.302\pm0.202$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-23$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J050006.39$+$010946.9 & $-0.852$ & $-0.613$ & $-0.613$ & $-0.162$ \\
J053504.12$-$341752.1 & $-1.166$ & $\dots$ & $\dots$ & $\dots$ \\
J063452.21$-$442544.3 & $-1.298$ & $\dots$ & $\dots$ & $-0.166$ \\
J064118.48$-$382036.2 & $-1.333$ & $\dots$ & $\dots$ & $\dots$ \\
J095934.05$+$370837.2 & $-1.548$ & $-0.517$ & $-0.517$ & $-0.150$ \\
J171855.25$+$383904.7 & $-0.825$ & $-0.128$ & $-0.128$ & $+0.015$ \\
J172831.49$-$694544.5 & $-0.979$ & $+0.242$ & $+0.252$ & $+0.259$ \\
J230156.02$-$410843.4 & $-0.842$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.095\pm0.265$ & $-0.283\pm0.367$ & $-0.283\pm0.371$ & $-0.159\pm0.015$\\
\multicolumn{5}{c}{$DTG-24$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J153604.92$+$024730.0 & $-2.670$ & $+0.362$ & $+0.662$ & $\dots$ \\
J173036.97$+$042141.4 & $-2.596$ & $-0.239$ & $+0.501$ & $+0.467$ \\
J173720.32$-$594017.3 & $-2.390$ & $\dots$ & $\dots$ & $\dots$ \\
J201052.13$-$472935.4 & $-1.679$ & $+0.293$ & $+0.343$ & $+0.226$ \\
J201243.95$-$240745.6 & $-2.563$ & $+0.084$ & $+0.614$ & $+0.504$ \\
J203337.10$-$501731.3 & $-2.040$ & $\dots$ & $\dots$ & $\dots$ \\
J204409.72$-$294009.3 & $-2.245$ & $+0.186$ & $+0.476$ & $+0.168$ \\
J211129.73$-$410133.2 & $-2.558$ & $+0.089$ & $+0.409$ & $+0.370$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.448\pm0.308$ & $+0.158\pm0.198$ & $+0.498\pm0.115$ & $+0.351\pm0.138$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-25$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: 2126804793521418112  (GL-1: \citet{Li2019})} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J024258.64$-$370938.0 & $-1.948$ & $+0.480$ & $+0.490$ & $+0.071$ \\
J035909.72$-$705241.7 & $-2.015$ & $+0.026$ & $+0.036$ & $+0.143$ \\
J114858.16$-$470406.2 & $-2.760$ & $\dots$ & $\dots$ & $\dots$ \\
J124353.25$-$385331.4 & $-2.680$ & $\dots$ & $\dots$ & $\dots$ \\
J142747.05$-$465910.2 & $-2.160$ & $\dots$ & $\dots$ & $\dots$ \\
J145041.74$+$665256.3 & $-2.781$ & $-0.188$ & $+0.492$ & $+0.551$ \\
J153639.20$-$652733.3 & $-2.406$ & $-0.170$ & $+0.480$ & $\dots$ \\
J192800.43$+$461406.8 & $-2.020$ & $-0.023$ & $+0.357$ & $+0.410$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.334\pm0.355$ & $-0.026\pm0.236$ & $+0.487\pm0.012$ & $+0.289\pm0.207$\\
\multicolumn{5}{c}{$DTG-26$} \\
\multicolumn{5}{c}{Structure: Thamnos} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J031356.38$-$655409.5 & $-2.398$ & $+0.841$ & $+0.861$ & $+0.226$ \\
J105829.62$+$001112.5 & $-3.212$ & $+0.771$ & $+0.781$ & $+0.282$ \\
J121528.31$-$345222.0 & $-2.440$ & $-0.327$ & $+0.143$ & $+0.549$ \\
J135443.70$-$340927.5 & $-1.640$ & $\dots$ & $\dots$ & $\dots$ \\
J144259.15$-$730508.1 & $-2.470$ & $\dots$ & $\dots$ & $\dots$ \\
J163038.75$+$132951.3 & $-1.861$ & $+0.103$ & $+0.273$ & $+0.307$ \\
J184634.34$-$762918.9 & $-2.350$ & $\dots$ & $\dots$ & $\dots$ \\
J212328.32$-$532829.1 & $-1.358$ & $+0.133$ & $+0.153$ & $+0.314$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.261\pm0.599$ & $+0.287\pm0.489$ & $+0.285\pm0.412$ & $+0.290\pm0.046$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-27$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Monty2020}} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J051340.78$-$062940.5 & $-2.426$ & $+0.002$ & $+0.672$ & $+0.213$ \\
J054143.88$-$724640.4 & $-2.200$ & $\dots$ & $\dots$ & $\dots$ \\
J064621.00$-$574119.3 & $-1.690$ & $\dots$ & $\dots$ & $\dots$ \\
J073958.20$+$131153.6 & $-1.734$ & $+0.067$ & $+0.097$ & $+0.500$ \\
J115256.91$-$444645.0 & $-1.800$ & $\dots$ & $\dots$ & $\dots$ \\
J155712.32$-$315003.9 & $-2.620$ & $\dots$ & $\dots$ & $\dots$ \\
J205802.68$+$142704.0 & $-2.061$ & $-0.349$ & $+0.031$ & $-0.196$ \\
J224253.45$+$365634.3 & $-1.789$ & $-0.299$ & $+0.111$ & $+0.508$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.991\pm0.352$ & $-0.145\pm0.191$ & $+0.083\pm0.049$ & $+0.337\pm0.312$\\
\multicolumn{5}{c}{$DTG-28$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Comoving: \citet{Myeong2017}} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: Ryu~879~(RLGC~2): \citet{Vasiliev2021}} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J050018.09$-$373529.0 & $-1.812$ & $+0.325$ & $+0.325$ & $+0.249$ \\
J051038.71$-$470902.9 & $-2.320$ & $\dots$ & $\dots$ & $\dots$ \\
J080900.33$+$285008.2 & $-2.666$ & $+0.121$ & $+0.471$ & $+0.464$ \\
J121001.39$+$452056.2 & $-2.526$ & $+0.039$ & $+0.149$ & $+0.331$ \\
J132722.65$-$165145.1 & $-1.590$ & $+0.256$ & $+0.296$ & $\dots$ \\
J150258.83$+$453916.0 & $-2.295$ & $-0.284$ & $+0.196$ & $+0.407$ \\
J201918.03$-$255201.7 & $-1.730$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.157\pm0.436$ & $+0.121\pm0.219$ & $+0.285\pm0.116$ & $+0.365\pm0.085$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-29$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J133847.37$-$421836.6 & $-2.700$ & $\dots$ & $\dots$ & $\dots$ \\
J150508.40$+$070154.5 & $-1.716$ & $-0.346$ & $-0.066$ & $+0.448$ \\
J151423.94$+$261334.2 & $-2.317$ & $-0.328$ & $+0.242$ & $+0.479$ \\
J161330.16$-$202216.3 & $-1.430$ & $\dots$ & $\dots$ & $\dots$ \\
J180749.18$-$545519.0 & $-2.460$ & $\dots$ & $\dots$ & $\dots$ \\
J183034.83$-$380055.9 & $-1.833$ & $-0.136$ & $+0.344$ & $\dots$ \\
J211251.73$+$211032.6 & $-2.533$ & $-0.131$ & $+0.569$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.179\pm0.492$ & $-0.235\pm0.108$ & $+0.283\pm0.241$ & $+0.464\pm0.016$\\
\multicolumn{5}{c}{$DTG-30$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J022714.83$+$634447.2 & $-1.062$ & $-0.303$ & $-0.303$ & $-0.030$ \\
J033657.79$+$291716.8 & $-1.037$ & $-0.361$ & $-0.341$ & $\dots$ \\
J040118.74$+$004217.1 & $-1.340$ & $-0.163$ & $-0.143$ & $-0.063$ \\
J073212.81$+$152358.6 & $-1.053$ & $-0.065$ & $-0.065$ & $-0.016$ \\
J114032.93$+$634044.0 & $-0.906$ & $+0.078$ & $+0.078$ & $+0.127$ \\
J130249.07$-$460903.1 & $-1.333$ & $+0.411$ & $+0.411$ & $\dots$ \\
J215506.12$-$663124.8 & $-1.055$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.052\pm0.016$ & $-0.095\pm0.265$ & $-0.086\pm0.259$ & $-0.035\pm0.053$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-31$} \\
\multicolumn{5}{c}{Structure: Splashed Disk} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J032816.91$-$780110.5 & $-0.847$ & $\dots$ & $\dots$ & $\dots$ \\
J065358.29$-$590948.0 & $-0.920$ & $\dots$ & $\dots$ & $\dots$ \\
J144436.77$+$393922.4 & $-1.077$ & $-0.479$ & $-0.479$ & $+0.243$ \\
J145903.10$+$054402.8 & $-1.032$ & $-0.159$ & $-0.159$ & $+0.598$ \\
J161651.70$-$094015.4 & $-1.200$ & $\dots$ & $\dots$ & $\dots$ \\
J202612.02$-$151201.4 & $-1.009$ & $\dots$ & $\dots$ & $\dots$ \\
J231223.21$-$462509.1 & $-0.930$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-0.999\pm0.113$ & $-0.319\pm0.168$ & $-0.319\pm0.168$ & $+0.420\pm0.187$\\
\multicolumn{5}{c}{$DTG-32$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J105249.35$-$070844.6 & $-0.927$ & $\dots$ & $\dots$ & $\dots$ \\
J120306.72$-$353748.3 & $-1.080$ & $\dots$ & $\dots$ & $\dots$ \\
J133030.29$-$155143.0 & $-0.990$ & $\dots$ & $\dots$ & $\dots$ \\
J153453.50$+$561024.4 & $-1.138$ & $+0.277$ & $+0.277$ & $+0.513$ \\
J210802.34$+$183540.2 & $-1.040$ & $-0.244$ & $-0.244$ & $-0.057$ \\
J212953.15$-$543412.9 & $-1.530$ & $\dots$ & $\dots$ & $\dots$ \\
J214820.59$+$215522.1 & $-0.909$ & $-0.188$ & $-0.188$ & $+0.013$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.024\pm0.155$ & $-0.215\pm0.067$ & $-0.215\pm0.067$ & $-0.021\pm0.148$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-33$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: NGC~6284: \citet{Vasiliev2021}} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J134415.78$-$414635.5 & $-2.450$ & $\dots$ & $\dots$ & $\dots$ \\
J143552.70$-$754824.8 & $-1.700$ & $\dots$ & $\dots$ & $\dots$ \\
J163318.77$-$770935.0 & $-2.880$ & $\dots$ & $\dots$ & $\dots$ \\
J165922.12$-$715018.9 & $-2.470$ & $\dots$ & $\dots$ & $\dots$ \\
J202309.64$-$152346.2 & $-2.300$ & $\dots$ & $\dots$ & $\dots$ \\
J210237.52$-$531613.3 & $-3.016$ & $+0.210$ & $+0.220$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.491\pm0.443$ & $+0.210\pm0.000$ & $+0.220\pm0.000$ & $\dots$\\
\multicolumn{5}{c}{$DTG-34$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: Sequoia: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Group Assoc: DTG-22: \citet{Limberg2021a}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: Ryu~879~(RLGC~2): \citet{Vasiliev2021}} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J020916.23$-$282501.4 & $-2.420$ & $-0.222$ & $+0.488$ & $-0.034$ \\
J080227.02$+$255154.6 & $-2.245$ & $+0.503$ & $+0.513$ & $+0.190$ \\
J115938.02$+$292211.4 & $-2.389$ & $-0.414$ & $+0.326$ & $+0.484$ \\
J142235.83$+$404556.8 & $-3.041$ & $+0.733$ & $+0.743$ & $+0.306$ \\
J173353.49$+$181556.6 & $-2.305$ & $+0.271$ & $+0.631$ & $+0.245$ \\
J174529.11$+$054921.1 & $-2.681$ & $-0.783$ & $-0.483$ & $+0.536$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.412\pm0.257$ & $+0.020\pm0.558$ & $+0.537\pm0.244$ & $+0.290\pm0.198$\\
\multicolumn{5}{c}{$DTG-35$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: NGC~5139~(oCen): \citet{Vasiliev2021}} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J180452.99$-$554355.1 & $-2.456$ & $+0.260$ & $+0.650$ & $+0.383$ \\
J184048.40$-$590443.9 & $-2.000$ & $\dots$ & $\dots$ & $\dots$ \\
J191455.63$-$502951.3 & $-2.033$ & $+0.278$ & $+0.288$ & $\dots$ \\
J201914.28$-$540455.3 & $-1.560$ & $\dots$ & $\dots$ & $\dots$ \\
J202313.18$-$072850.4 & $-2.539$ & $+0.791$ & $+1.161$ & $+0.016$ \\
J214250.04$-$620156.3 & $-1.810$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.058\pm0.358$ & $+0.269\pm0.016$ & $+0.690\pm0.374$ & $+0.200\pm0.193$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-36$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J061416.29$-$475943.7 & $-1.620$ & $\dots$ & $\dots$ & $\dots$ \\
J084908.87$+$041323.9 & $-1.260$ & $\dots$ & $\dots$ & $\dots$ \\
J100801.43$-$415047.5 & $-1.611$ & $-0.205$ & $-0.165$ & $+0.144$ \\
J114234.79$-$472538.4 & $-1.920$ & $\dots$ & $\dots$ & $\dots$ \\
J230958.05$-$580926.2 & $-1.190$ & $\dots$ & $\dots$ & $\dots$ \\
J232938.45$+$333709.6 & $-2.962$ & $+0.059$ & $+0.449$ & $+0.394$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.607\pm0.545$ & $-0.073\pm0.139$ & $+0.142\pm0.323$ & $+0.269\pm0.132$\\
\multicolumn{5}{c}{$DTG-37$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J171436.22$-$672612.5 & $-2.812$ & $-0.247$ & $+0.383$ & $+0.412$ \\
J172851.63$-$694103.8 & $-2.419$ & $+0.266$ & $+0.716$ & $+0.106$ \\
J174734.65$-$734946.6 & $-2.650$ & $\dots$ & $\dots$ & $\dots$ \\
J202352.24$-$162851.2 & $-2.714$ & $-0.109$ & $+0.611$ & $+0.188$ \\
J210115.04$-$434751.5 & $-2.293$ & $-0.306$ & $+0.004$ & $+0.150$ \\
J220841.10$-$394512.2 & $-2.381$ & $+0.311$ & $+0.391$ & $+0.157$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.542\pm0.201$ & $-0.041\pm0.290$ & $+0.426\pm0.255$ & $+0.151\pm0.040$\\
\multicolumn{5}{c}{$DTG-38$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J030446.60$+$483710.9 & $-1.228$ & $-0.165$ & $-0.165$ & $+0.088$ \\
J031409.77$+$114351.2 & $-0.928$ & $+0.007$ & $+0.007$ & $+0.176$ \\
J052613.64$-$040946.3 & $-1.433$ & $-0.242$ & $-0.242$ & $-0.074$ \\
J223215.63$-$485715.7 & $-1.137$ & $\dots$ & $\dots$ & $\dots$ \\
J235457.16$-$214223.0 & $-0.954$ & $+0.392$ & $+0.392$ & $+0.396$ \\
J235500.07$+$125504.2 & $-1.281$ & $-0.072$ & $-0.072$ & $+0.120$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.163\pm0.187$ & $-0.100\pm0.204$ & $-0.100\pm0.204$ & $+0.110\pm0.165$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-39$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: CDTG-14: \citet{Gudin2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J022151.19$-$593331.9 & $-2.340$ & $\dots$ & $\dots$ & $\dots$ \\
J155551.34$+$125605.4 & $-2.032$ & $-0.122$ & $+0.218$ & $+0.491$ \\
J163114.30$-$001305.5 & $-1.950$ & $\dots$ & $\dots$ & $\dots$ \\
J171349.03$+$464333.4 & $-2.705$ & $+0.132$ & $+0.332$ & $+0.379$ \\
J200228.85$-$533114.4 & $-3.100$ & $\dots$ & $\dots$ & $\dots$ \\
J220136.69$-$691831.2 & $-1.936$ & $-0.145$ & $+0.105$ & $+0.211$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.241\pm0.467$ & $-0.133\pm0.020$ & $+0.218\pm0.095$ & $+0.364\pm0.121$\\
\multicolumn{5}{c}{$DTG-40$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J123258.46$-$325442.0 & $-2.344$ & $-0.115$ & $+0.575$ & $\dots$ \\
J131549.29$-$140429.0 & $-2.189$ & $-0.429$ & $-0.319$ & $+0.373$ \\
J132604.50$-$152502.0 & $-1.890$ & $\dots$ & $\dots$ & $\dots$ \\
J204309.47$-$360032.6 & $-2.279$ & $+0.575$ & $+0.635$ & $+0.381$ \\
J215746.83$-$030301.9 & $-2.130$ & $\dots$ & $\dots$ & $\dots$ \\
J231431.40$-$773532.0 & $-3.160$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.195\pm0.194$ & $-0.033\pm0.457$ & $+0.604\pm0.053$ & $+0.377\pm0.004$\\
\multicolumn{5}{c}{$DTG-41$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J022004.14$-$350533.3 & $-1.742$ & $-0.048$ & $+0.262$ & $+0.288$ \\
J022655.73$-$395753.7 & $-2.014$ & $-0.139$ & $+0.391$ & $+0.356$ \\
J044117.84$-$494021.0 & $-1.610$ & $\dots$ & $\dots$ & $\dots$ \\
J102607.52$-$443036.1 & $-2.268$ & $+0.536$ & $+0.836$ & $\dots$ \\
J130730.29$+$494834.7 & $-2.573$ & $-0.165$ & $+0.405$ & $+0.400$ \\
J204611.88$-$383311.8 & $-1.471$ & $+0.012$ & $+0.032$ & $+0.188$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.925\pm0.403$ & $-0.083\pm0.155$ & $+0.359\pm0.281$ & $+0.315\pm0.085$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-42$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Monty2020}} \\
\multicolumn{5}{c}{Group Assoc: Sausage: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J054348.06$-$253841.7 & $-1.504$ & $+0.206$ & $+0.226$ & $+0.172$ \\
J083925.07$-$731740.0 & $-1.990$ & $\dots$ & $\dots$ & $\dots$ \\
J091626.88$-$642359.4 & $-1.440$ & $\dots$ & $\dots$ & $\dots$ \\
J110013.27$-$131258.2 & $-2.270$ & $+0.448$ & $+0.458$ & $+0.214$ \\
J172738.86$-$513330.0 & $-2.139$ & $-0.255$ & $+0.425$ & $\dots$ \\
J185121.35$+$531911.5 & $-1.637$ & $+0.326$ & $+0.346$ & $+0.060$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.826\pm0.333$ & $+0.278\pm0.271$ & $+0.377\pm0.096$ & $+0.159\pm0.072$\\
\multicolumn{5}{c}{$DTG-43$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J120455.05$-$400546.2 & $-1.471$ & $+0.109$ & $+0.129$ & $+0.325$ \\
J123044.46$-$723618.9 & $-1.476$ & $-0.247$ & $-0.097$ & $\dots$ \\
J171754.94$-$631654.2 & $-1.774$ & $+0.166$ & $+0.226$ & $+0.457$ \\
J183524.81$-$363914.0 & $-1.956$ & $+1.007$ & $+1.027$ & $+0.052$ \\
J195404.66$-$871428.7 & $-2.280$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.782\pm0.316$ & $+0.108\pm0.477$ & $+0.113\pm0.392$ & $+0.293\pm0.183$\\
\multicolumn{5}{c}{$DTG-44$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J063828.90$-$830931.9 & $-2.474$ & $+0.020$ & $+0.440$ & $+0.265$ \\
J170501.04$-$705240.7 & $-1.816$ & $+0.235$ & $+0.245$ & $+0.643$ \\
J175726.75$-$491934.8 & $-1.700$ & $\dots$ & $\dots$ & $\dots$ \\
J200709.43$-$041721.3 & $-1.379$ & $+0.097$ & $+0.117$ & $+0.369$ \\
J224408.15$-$333118.5 & $-1.650$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.661\pm0.284$ & $+0.112\pm0.095$ & $+0.263\pm0.140$ & $+0.400\pm0.177$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-45$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: DTG-10: \citet{Limberg2021a}} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J050146.92$+$030030.6 & $-1.574$ & $-0.185$ & $-0.185$ & $-0.074$ \\
J063058.49$-$575741.3 & $-2.180$ & $-0.433$ & $+0.287$ & $\dots$ \\
J083704.03$+$783015.9 & $-2.553$ & $+0.426$ & $+0.696$ & $+0.358$ \\
J150312.86$+$060215.6 & $-1.953$ & $-0.003$ & $+0.117$ & $+0.335$ \\
J221329.39$-$021012.3 & $-0.916$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.893\pm0.590$ & $-0.074\pm0.333$ & $+0.216\pm0.336$ & $+0.346\pm0.020$\\
\multicolumn{5}{c}{$DTG-46$} \\
\multicolumn{5}{c}{Structure: Gaia-Sausage-Enceladus (GSE)} \\
\multicolumn{5}{c}{Group Assoc: DTG-38: \citet{Limberg2021a}} \\
\multicolumn{5}{c}{Stellar Assoc: J173145.54+284315.7 (DTG-14: \citet{Yuan2020b})} \\
\multicolumn{5}{c}{Globular Assoc: UKS~1: \citet{Vasiliev2021}} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J054233.11$-$591339.8 & $-1.621$ & $+0.329$ & $+0.359$ & $+0.083$ \\
J091710.78$-$614706.7 & $-2.371$ & $+0.232$ & $+0.452$ & $-0.015$ \\
J163420.44$+$115756.4 & $-2.181$ & $+0.569$ & $+0.579$ & $+0.533$ \\
J173145.52$+$284315.4 & $-2.146$ & $+0.418$ & $+0.428$ & $+0.163$ \\
J195126.62$-$501322.4 & $-1.710$ & $-0.224$ & $-0.094$ & $+0.151$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.038\pm0.337$ & $+0.372\pm0.247$ & $+0.448\pm0.125$ & $+0.107\pm0.162$\\
\multicolumn{5}{c}{$DTG-47$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J000403.11$-$610636.8 & $-1.270$ & $-0.607$ & $-0.607$ & $-0.185$ \\
J030400.59$+$273824.6 & $-0.818$ & $-0.310$ & $-0.310$ & $+0.072$ \\
J044249.06$+$182159.8 & $-1.075$ & $-0.070$ & $-0.070$ & $+0.319$ \\
J070149.11$+$231847.4 & $-1.523$ & $-0.374$ & $-0.374$ & $-0.055$ \\
J114011.83$-$791820.6 & $-0.830$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.093\pm0.280$ & $-0.341\pm0.200$ & $-0.341\pm0.200$ & $+0.022\pm0.198$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-48$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J025648.05$-$194247.2 & $-0.940$ & $\dots$ & $\dots$ & $\dots$ \\
J032305.19$+$004104.1 & $-1.510$ & $\dots$ & $\dots$ & $\dots$ \\
J032425.19$-$155005.4 & $-2.050$ & $\dots$ & $\dots$ & $\dots$ \\
J040732.19$-$150818.1 & $-1.447$ & $-0.249$ & $-0.249$ & $-0.061$ \\
J043636.11$-$174723.7 & $-0.843$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.360\pm0.456$ & $-0.249\pm0.000$ & $-0.249\pm0.000$ & $-0.061\pm0.000$\\
\multicolumn{5}{c}{$DTG-49$} \\
\multicolumn{5}{c}{Structure: Metal-Weak Thick Disk (MWTD)} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J022151.61$+$474350.2 & $-1.041$ & $-0.133$ & $-0.133$ & $+0.031$ \\
J055625.55$-$171842.6 & $-1.313$ & $\dots$ & $\dots$ & $\dots$ \\
J072846.92$+$814943.7 & $-2.692$ & $+0.507$ & $+0.767$ & $+0.424$ \\
J074003.26$-$074058.8 & $-2.385$ & $+0.006$ & $+0.456$ & $+0.431$ \\
J225344.78$-$545648.6 & $-1.488$ & $+0.293$ & $+0.303$ & $+0.341$ \\
$\mu \pm \sigma$ ([X/Y]) & $-1.690\pm0.740$ & $+0.163\pm0.263$ & $+0.365\pm0.342$ & $+0.398\pm0.073$\\
\multicolumn{5}{c}{$DTG-50$} \\
\multicolumn{5}{c}{Structure: Unassigned Structure} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: 6083718580940298624 (NGC~5139~(oCen): \citet{Vasiliev2021})} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J132539.03$-$471827.1 & $-2.180$ & $\dots$ & $\dots$ & $\dots$ \\
J144604.01$-$730314.2 & $-2.336$ & $-0.569$ & $+0.121$ & $+0.043$ \\
J195521.57$-$461357.1 & $-2.519$ & $+0.337$ & $+0.757$ & $-0.088$ \\
J200810.50$-$834659.9 & $-1.968$ & $-0.271$ & $-0.061$ & $+0.075$ \\
J230047.40$-$724311.9 & $-2.185$ & $+0.137$ & $+0.147$ & $+0.486$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.227\pm0.196$ & $-0.084\pm0.372$ & $+0.078\pm0.255$ & $+0.025\pm0.201$\\
\pagebreak \\[-3.5ex]
\multicolumn{5}{c}{$DTG-51$} \\
\multicolumn{5}{c}{Structure: Thamnos} \\
\multicolumn{5}{c}{Group Assoc: GL-4: \citet{Li2019}} \\
\multicolumn{5}{c}{Group Assoc: SeqG1: \citet{Monty2020}} \\
\multicolumn{5}{c}{Group Assoc: Sequoia: \citet{Cordoni2021}} \\
\multicolumn{5}{c}{Group Assoc: DTG-31: \citet{Limberg2021a}} \\
\multicolumn{5}{c}{Stellar Assoc: J122218.69-385337.0 (Sequoia: \citet{Cordoni2021})} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J122218.68$-$385336.9 & $-2.710$ & $+0.494$ & $+0.504$ & $+0.112$ \\
J133730.08$-$771750.0 & $-2.732$ & $+0.407$ & $+0.447$ & $+0.096$ \\
J161727.40$-$154918.2 & $-2.320$ & $\dots$ & $\dots$ & $\dots$ \\
J231316.39$-$701122.5 & $-2.460$ & $+0.311$ & $+0.491$ & $\dots$ \\
J234954.26$-$570852.8 & $-1.380$ & $\dots$ & $\dots$ & $\dots$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.485\pm0.451$ & $+0.404\pm0.077$ & $+0.488\pm0.028$ & $+0.104\pm0.008$\\
\multicolumn{5}{c}{$DTG-52$} \\
\multicolumn{5}{c}{Structure: Helmi Stream} \\
\multicolumn{5}{c}{Group Assoc: No Group Associations} \\
\multicolumn{5}{c}{Stellar Assoc: No Stellar Associations} \\
\multicolumn{5}{c}{Globular Assoc: No Globular Associations} \\
\multicolumn{5}{c}{Dwarf Galaxy Assoc: No Dwarf Galaxy Associations} \\
J031559.17$-$381317.6 & $-1.971$ & $-0.443$ & $+0.117$ & $+0.309$ \\
J081308.63$+$392556.2 & $-2.479$ & $-0.440$ & $+0.160$ & $+0.496$ \\
J085716.00$-$655611.2 & $-2.642$ & $+0.468$ & $+0.478$ & $+0.191$ \\
J141759.95$-$241546.3 & $-2.535$ & $+0.161$ & $+0.791$ & $\dots$ \\
J172347.39$-$583412.5 & $-2.004$ & $-0.210$ & $+0.280$ & $+0.026$ \\
$\mu \pm \sigma$ ([X/Y]) & $-2.396\pm0.347$ & $-0.146\pm0.393$ & $+0.322\pm0.261$ & $+0.253\pm0.180$\\
\enddata
\end{deluxetable*}

